Sample and Threshold Differential Privacy: Histograms and applications

Federated analytics seeks to compute accurate statistics from data distributed across users' devices while providing a suitable privacy guarantee and being practically feasible to implement and scale. In this paper, we show how a strong $(\epsilon, \delta)$-Differential Privacy (DP) guarantee can be achieved for the fundamental problem of histogram generation in a federated setting, via a highly practical sampling-based procedure that does not add noise to disclosed data. Given the ubiquity of sampling in practice, we thus obtain a DP guarantee almost for free, avoid over-estimating histogram counts, and allow easy reasoning about how privacy guarantees may obscure minorities and outliers. Using such histograms, related problems such as heavy hitters and quantiles can be answered with provable error and privacy guarantees. Experimental results show that our sample-and-threshold approach is accurate and scalable.

==> cut.tex <==

\section{Analysis of original TrieHH protocol}

We adopt the algorithm and notation from the TrieHH paper~\cite{TrieHH}. 

The algorithm proceeds over $L$ levels. 
At each level, we sample $m = \gamma \sqrt{n}$ clients to report on their items that extend the current trie. 
We add items to the current trie based on an (absolute) threshold $\threshold$. 


\subsection{Simplification of \cite[Lemma 2]{TrieHH}}

Lemma 2 in~\cite{TrieHH} considers the difference in probabilities between inputs $D$ and $D'$
for reporting a particular prefix.
The set up is that there are $k$ users in $D'$ who hold the prefix, but $k+1$ in $D$. 

\begin{lemma}
Given the set up above, with $k+1 \leq \sqrt{n}/\gamma$, 
the probability of reporting the prefix is at most
$\exp(-\threshold \ln \threshold + \threshold - 1)$ for any $\threshold > 1$.
\label{lem:ptheta}
\end{lemma}

\begin{proof}
The algorithm will report the prefix if the number of sampled occurrences is at least $\threshold$. 
We analyze the case of sampling the clients with replacement.  
Note that this only increases the chances of this event. 

The probability of picking the prefix in one sample is just
$p:= (k+1)/n \leq 1/m$.  
Let $X$ denote the random variable with the number of successes (times the prefix is picked) out of the $m$ trials. 
We have 
\[ \E[X] = \frac{m(k+1)}{n} \leq \frac{m \sqrt{n}}{\gamma n} = 1\] 
using the bound on $k+1$, and the fact that $m = \gamma \sqrt{n}$. 
Then, 
%$\Var[X] \leq \E[X] = 1$ since 
$X$ is a sum of $m$ Bernoulli random variables with $p \leq 1/m$. 

We then apply a Chernoff-Hoeffding bound to the mean of the $m$ trials: 

\[ \Pr[ X \ge \threshold ] = \Pr\left[ \frac{1}{m}X - \frac{1}{m}\E[X] \ge \left(\frac{\threshold}{m} - \frac{1}{m}\right) \right] \le 
%\exp(- (\threshold-1)^2/ 3)
\exp\left(- D\left( \frac{\threshold}{m} \middle\| \frac{1}{m}\right)m\right) . 
%\exp\left( - \frac{(\threshold-1)^2}{\threshold +1}\right) .
%\le  \textstyle \exp( - \frac{1}{2}(\threshold-1)^2) . 
\]

Here, $D(p\|q)$ denotes the K-L divergence (relative entropy) between the (Bernoulli) distributions with parameters $p$ and $q$. 
We have
\begin{align*}
-D(p\|q) m  & = -{\threshold} \ln\left(\frac{\threshold}{m} \cdot \frac{m}{1}\right) - {m-\threshold}\ln\left(\frac{m - \threshold}{m} \cdot \frac{m}{m-1}\right)
\\
& =  {-\threshold} \ln \threshold - (m-\threshold) \ln\left(1 - \frac{\threshold-1}{m-1}\right)\\
& = -\threshold \ln \threshold + (m-\threshold) \ln\left( \frac{m-1}{m -\threshold}\right) \\
& = -\threshold \ln \threshold + (m-\threshold) \ln \left(1 + \frac{\threshold-1}{m-\threshold}\right) \\
& \leq - \threshold \ln\threshold + \threshold - 1
\end{align*}

\begin{equation}
\text{Hence, }
  \Pr[ X \ge \threshold ] \leq \exp(-\threshold \ln \threshold + \threshold - 1)
\end{equation}
\end{proof}


In contrast, the result proved in~\cite{TrieHH} is a bound of 
$\frac{\threshold-2}{\threshold-3} \frac{1}{\threshold!}$. 
The expression in Lemma~\ref{lem:ptheta} is slightly looser. 

To achieve a target error bound $\delta$, we rearrange to obtain
$\frac{\threshold}{e} \ln \frac{\threshold}{e}  = \frac{1}{e} \ln(1/e\delta)$, and apply Lambert's W function. 
This gives 
$\frac{\threshold}{e} = W(\frac{1}{e} \ln(1/e\delta)$, i.e., 
$\threshold = e W(\frac{1}{e} \ln \frac{1}{e\delta})$. 


\subsection{Short version of \cite[Lemma 1]{TrieHH}}

We next give a short version of a bound on the ratio of probabilities of seeing the same output on neighboring inputs. 
This follows the same proof outline as in the original paper. 

\begin{proof}
The case to focus on is when input $D$ has one extra copy of a particular prefix compared to $D'$, at some intermediate stage of the algorithm. 
Without loss of generality, we can imagine that this copy is held by the user with index $n$. 
%
For notation, we will write 
%$C(n, k)$ to be the number of ways to choose $k$ items from a collection of $n$ (i.e., this is just $n \choose k$), and we 
%will write 
$S_k(n, m, \threshold)$ to denote the number of ways to succeed in collecting at least $\threshold$ instances of the target prefix while picking $m$ items out of $n$, when there are $k$ total instances of the prefix. 

For $D'$, we can break their successful instances into (a) those where they sample item $n$ and need to collect $\threshold$ instances with their remaining $m-1$ samples out of $n-1$ items, or (b) where they do not sample item $n$, and thus need to collect $\threshold$ instances from $m$ samples out of $n$. Thus, 
\begin{equation}
S_k(n, m, \threshold) = S_k(n-1, m, \threshold) + S_k(n-1, m-1, \threshold)
\label{eq:dprime}
\end{equation}

For $D$, we first derive a useful relationship that corresponds to the case that $D$ does not pick index $n$. 
This is equivalent to considering their success on a smaller instance without the $n$'th item. 
$D$ will succeed if they pick exactly $\threshold$ instances of the target prefix from the $k$ instances
(and $m-\threshold$ from any of the remaining $n-1-k$ items), or pick more than $\threshold$.
We can express this in our notation as
\[ S_{k}(n-1, m, \threshold) = {k \choose \threshold} {n-k-1 \choose m-\threshold} + S_k(n-1, m, \threshold+1)
\]

Rearranging, we obtain that
\[ {n-k-1 \choose m - \threshold} \leq  {k \choose \threshold}^{-1} S_{k}(n-1, m, \threshold)
\]

The set of routes to success for $D$ look similar to those for $D'$, with one extra case: 
(a) $D$ does not pick item $n$, and succeeds with $m$ samples over the $n-1$ remaining items;
(b) $D$ does pick $n$, and picks $\threshold$ or more items from the remaining $n-1$;
(c) or else $D$ picks index $n$ and exactly $\threshold-1$ copies of the target prefix from among the 
$k$ copies, along with $m - \threshold$ from the remaining $(n-1) - k$ items. 
This gives
\begin{align*}
    S_{k+1}(n, m, \threshold) & =  S_k(n-1, m, \threshold) + S_k(n-1, m-1, \threshold) + {k \choose \threshold-1} {n-k-1 \choose m-\threshold} \\
    & \leq  S_k(n-1, m, \threshold) + S_k(n-1, m-1, \threshold) + {{k \choose \threshold-1}\over {k \choose \threshold}} S_k(n-1, m, \threshold) \\
    & =  S_k(n-1, m-1, \threshold) + \left(1 + \frac{\threshold}{k - \threshold +1}\right)S_k(n-1, m, \threshold)\\
    & \leq  \left(1 + \frac{\threshold}{k-\threshold+1}\right)S_k(n, m, \threshold) 
\end{align*}

\noindent
where the last line follows from \eqref{eq:dprime}.

This determines the critical ratio $S_{k+1}(n,m, \threshold)/S_k(n, m, \threshold) \leq \frac{k+1}{k-\threshold+1}$, as required, which is the ratio between the seeing the prefix appear in the output of $D$ versus that of $D'$. 
\end{proof}




\subsection{Simplification of \cite[Corollary 1]{TrieHH}}

We consider the proof of the main technical result in~\cite{TrieHH}. 

\cite[Lemma~1]{TrieHH} shows that the ratio of probabilities of seeing outputs at level $i$ is bounded by a factor of 
$(1 + \frac{\threshold}{k - \threshold + 1})$, for $k \geq \threshold$. 
This is used to prove the main bound in \cite[Theorem 1]{TrieHH}. 
The proof of \cite[Theorem 1]{TrieHH} proceeds by considering the accumulated probability of different outcomes, based on a case split 
for when the probability of a certain event falls below $p_\threshold$. 
In the proof, $p_\threshold$ is set to $\frac{\threshold-2}{\threshold-3} \frac{1}{\threshold!}$, to agree with the bound proved in \cite[Lemma 2]{TrieHH}. 
However, there is nothing in the proof that requires this particular value of $p_\threshold$, so we can follow the same proof argument, and obtain a restatement of \cite[Theorem 1]{TrieHH} as providing $(\epsilon, \delta)$-differential privacy
with $\epsilon = L \ln( 1 + \frac{1}{\frac{\sqrt{n}}{\gamma \threshold} - 1})$
and $\delta = \exp(-\threshold \ln \threshold)$. 

We will provide a simplified bound on the expression of $\epsilon$ to make it easier to work with.


First, observe that, with the assumption that $k \ge \sqrt{n}{\gamma} - 1 \ge \threshold$ and $m = \gamma n$,  
\begin{equation}
\label{eq:epsbound}    
1 + \frac{\threshold}{k-\threshold + 1}
\le 1 + \frac{\threshold}{\frac{n}{m} - \threshold}
= 1 + \frac{1}{\frac{n}{m\threshold} - 1}
%1 + \frac{1}{\frac{\sqrt{n}}{\gamma \threshold} - 1 } = 1 + \frac{1}{ \frac{n}{m\threshold} - 1}
 = 1 + \frac{m\threshold}{n - m\threshold} . 
\end{equation}
%\noindent
%using the fact that $m = \gamma \sqrt{n}$. 

We will assume that $\gamma \leq \frac{\sqrt{n}}{10\threshold}$. 
This is a stronger assumption that
\cite{TrieHH}, which assumes only
$\gamma \leq \frac{\sqrt{n}}{\threshold + 1}$. 
The effect is to ensure that the sample size $m$ is a small fraction of $n$. 
Substituting this assumption in \eqref{eq:epsbound}, we conclude 
\begin{equation}
    \label{eq:finalepsbound}
    1 + \frac{1}{\frac{\sqrt{n}}{\gamma \threshold} - 1 }  \leq 1 + \frac{m\threshold}{n - n/10}
    = 1 + \frac{10 m \threshold}{9n} 
\end{equation}

Since $\frac{10m\threshold}{9n} \leq 1$, we can bound
$\epsilon \leq \frac{10 L m \threshold}{9n}$. 

This form is a bit looser than the result in~\cite{TrieHH}.
%, but easier to manipulate. 
Specifically, given a target $(\epsilon, \delta)$, we can 
first use Lemma~\ref{lem:ptheta} to set
$\threshold = e \exp( W(\frac{1}{e}\ln(1/e\delta))$,\footnote{Recall, $W(\cdot)$ denotes the Lambert W-function.  
Since we only need to consider integral values of $\threshold$, we can also find $\threshold$ from 
$\delta$ with a small lookup table: 
$\threshold = 100$ gives $\delta = 10^{-157}$, which is likely to be small enough for all purposes. } and 
hence 
$m = \frac{9\epsilon}{10 L \threshold} n$.
%= \frac{9 \epsilon}{10 L \exp(W(\ln(1/\delta))}$. 

Interpreting this expression, we can treat $\threshold$ effectively as a small constant, and the main dependence is on 
$\epsilon/L$.  
This means for that stronger privacy, we should pick a smaller sample (giving a lower chance to learn information about any particular client). 
As we see below, this contrasts with the goal of accuracy, where we would prefer a larger sample to get more accurate results. 

Concretely, comparing to values computed in~\cite{TrieHH}, 
for $n = 10^{5}$, $\epsilon = 2$, $L=10$, and $\delta = 1/n^2$, 
we obtain
$\threshold = \lceil \exp(W(\ln(10^{-12}) \rceil = 14$, and
$m = (18/1400) n = 0.01285n$. 
Using the expression from~\cite{TrieHH} of
$m = \frac{1}{\threshold}(1 - \exp(-\epsilon/L)) n = 0.01293 n$, i.e., very close agreement. 

%Overall, this allows us to pick a smaller sample size $m$ (or $\gamma$) to achieve the same level of differential privacy, due to the tighter calculation of the threshold $\threshold$. 



\end{document}
